Semantic Calibration Prevails Where Token Confidence Fails: Benchmarking Long-Form Scientific QA

Reliable uncertainty quantification (UQ) is essential for safe deployment of large language models (LLMs) in scientific question answering, where long-form outputs exceed practical human verification at scale. We introduce the first large-scale benchmark for UQ calibration in long-form, reasoning-demanding scientific QA, evaluating four UQ methods on 685,000 responses across up to 20 LLMs and seven datasets, supported by an extensible open-source framework whose shared-generation design enables reproducible cross-method comparisons. Instruction tuning is shown to associate with systematic token probability polarization, collapsing confidence distributions and undermining the reliability of token-level uncertainty signals. Reasoning model families diverge: some reproduce this polarization while others actively mitigate it, a pattern that clusters by provider and suggests training pipeline design as a key differentiating factor. Verbalized and token-aggregation sequence-level methods fail systematically. Only semantic consistency, as measured by consistency of the final answer, yields well-calibrated outputs, providing the first large-scale evidence that semantic calibration persists in multi-step, dependency-rich reasoning settings.

==> preamble_iclr.tex <==
\usepackage{titlesec}
\titlespacing*{\section}
  {0pt}      % left indent
  {.75em}      % space before the section heading
  {.75em}    % space after the section heading
  
\titlespacing*{\subsection}
  {0pt}      % left indent
  {.5em}      % space before the section heading
  {.5em}    % space after the section heading
  
\titlespacing*{\paragraph}
  {0pt}      % left indent
  {.25em}      % space before the section heading
  {.25em}    % space after the section heading

\author{
Philip Müller \\
Helmholtz-Zentrum Dresden-Rossendorf \\ % https://orcid.org/0009-0005-5986-5628
\texttt{p.mueller@hzdr.de}
\And
Nicholas Popovič \\
Technische Universität Dresden \\
ScaDS.AI \\
\texttt{nicholas.popovic@tu-dresden.de}
\And
Michael Färber \\ 
Technische Universität Dresden \\
ScaDS.AI \\
\texttt{michael.faerber@tu-dresden.de}
\And
Peter Steinbach \\ % https://orcid.org/0000-0002-4974-230X
Helmholtz-Zentrum Dresden-Rossendorf \\
%Head, Group of Artificial Intelligence \\
\texttt{p.steinbach@hzdr.de}
}

\title{Benchmarking Uncertainty Estimation\\ in Large Language Model Replies\\ for Natural Science Question Answering}
%\iclrfinalcopy % - activate should the paper be accepted


==> tables/invalid_answers_struct_decoding.tex <==
\begin{table}[H]
\caption{\textbf{After Using Structured Decoding: Number of Invalid Answers Given by Models for Prompt 1 Across All Datasets (\(n = 25{,}316\)) After Experiment Adjustment.} We adjusted the experiment as a result of the behaviour described above to use structured decoding. The new resulting invalid answer counts are shown in this table. Due to the updated experiment leveraging structured decoding, invalid answers can only happen in reasoning model when the reasoning chains break the max token sampling parameter. The max token parameter in the updated experiment was set to 10.240 tokens (or higher depending on the configuration).}
\centering
\begin{tabularx}{\textwidth}{lrrrr}
\toprule
\textbf{Model} & \textbf{Prompt 1} & \textbf{Prompt 2} & \textbf{Prompt 3} & \textbf{Prompt 4} \\
\midrule
gpt-oss-20b & 307  & 3356  & 498   & 25304 \\
gpt-oss-120b & 38  & 3323  & 27    & 24873 \\
Ministral-8B-Instruct-2410 & 0    & 0     & 0     & 0 \\
Mistral-Nemo-Base-2407 & 0        & 0     & 12574 & 0 \\
Mistral-Nemo-Instruct-2407 & 0     & 0     & 0     & 0 \\
Mistral-Small-3.1-24B-Base-2503 & 0 & 0     & 0     & 0 \\
Mistral-Small-3.2-24B-Instruct-2506 & 0 & 0 & 0     & 0 \\
Magistral-Small-2507 & 0          & 0     & 0     & 0 \\
Magistral-Small-2507-Reasoning-Enabled & 8604 & 18716 & 4749 & 21232 \\
Llama-3.1-70B & 0                 & 13    & 0     & 6636 \\
Llama-3.3-70B-Instruct & 0        & 2527  & 19    & 125 \\
Llama-4-Scout-17B-16E & 2         & 3     & 0     & 5048 \\
Llama-4-Scout-17B-16E-Instruct & 0 & 15   & 0     & 0 \\
Qwen3-30B-A3B-Base & 2           & 1     & 0     & 55 \\
Qwen3-30B-A3B-Instruct-2507 & 0   & 6270  & 0     & 722 \\
Qwen3-30B-A3B-Thinking-2507 & 6242 & 11746 & 8656 & 21840 \\
DeepSeek-R1-Distill-Llama-70B & 425 & 7538 & 725  & 7477 \\
DeepSeek-R1-Distill-Qwen-32B & 914 & 7465 & 1170 & 3337 \\
gemma-3-27b-it & 0               & 431   & 0     & 2 \\
\bottomrule
\end{tabularx}

\label{tab:invalid_answers}
\end{table}
